UniRef++: Segment Every Reference Object in Spatial and Temporal Spaces

The reference-based object segmentation tasks, namely referring image segmentation (RIS), few-shot image segmentation (FSS), referring video object segmentation (RVOS), and video object segmentation (VOS), aim to segment a specific object by utilizing either language or annotated masks as references. Despite significant progress in each respective field, current methods are task-specifically designed and developed in different directions, which hinders the activation of multi-task capabilities for these tasks. In this work, we end the current fragmented situation and propose UniRef++ to unify the four reference-based object segmentation tasks with a single architecture. At the heart of our approach is the proposed UniFusion module which performs multiway-fusion for handling different tasks with respect to their specified references. And a unified Transformer architecture is then adopted for achieving instance-level segmentation. With the unified designs, UniRef++ can be jointly trained on a broad range of benchmarks and can flexibly complete multiple tasks at run-time by specifying the corresponding references. We evaluate our unified models on various benchmarks. Extensive experimental results indicate that our proposed UniRef++ achieves state-of-the-art performance on RIS and RVOS, and performs competitively on FSS and VOS with a parameter-shared network. Moreover, we showcase that the proposed UniFusion module could be easily incorporated into the current advanced foundation model SAM and obtain satisfactory results with parameter-efficient finetuning. Codes and models are available at \url{https://github.com/FoundationVision/UniRef}.

==> tables/ab_vl.tex <==
\begin{tabular}{cccc}
\toprule[1pt]

Variants & \mjf & \mj & \mf \\
\midrule

Sequential M-\textgreater L & 13.8 & 14.6 & 13.0 \\
Sequential L-\textgreater M & 9.5 & 9.6 & 9.5 \\
\rowcolor{lightgray!28}Parallel & 60.1 & 58.9 & 61.4 \\

\bottomrule[1pt]
\end{tabular}

==> tables/rec.tex <==
\begin{tabular}{l|l|l|c|c|c|c|c|c|c|c}
      \toprule[1pt]
      \multirow{2}{*}{Method} & Visual &
      Text & 
      \multicolumn{3}{c|}{RefCOCO}  & \multicolumn{3}{c|}{RefCOCO+} & \multicolumn{2}{c}{RefCOCOg} \\
      \cline{4-11}
                                    & Backbone & Encoder & val   & test A & test B & val & test A & test B & val-u & test-u  \\
      \hline
    %   MAttNet~\cite{yu2018mattnet} & RN101 & Bi-LSTM & 76.65 & 81.14 & 69.99 & 65.33 & 71.62 & 56.02 & 66.58 & 67.27 \\ 
      UNTIER-L~\cite{chen2020uniter} & RN101 & BERT & 81.41 & 87.04 & 74.17 & 75.90 & 81.45 & 66.70 & 74.86 & 75.77 \\
      VILLA-L~\cite{gan2020villa} & RN101 & BERT & 82.39 & 87.48 & 74.84 & 76.17 & 81.54 & 66.84 & 76.18 & 76.71 \\
      RefTR~\cite{li2021reftr} & RN101 & BERT-base & 85.65 & 88.73 & 81.16 & 77.55 & 82.26 & 68.99 & 79.25 & 80.01 \\ 
    SeqTR~\cite{zhu2022seqtr} & DN53 & Bi-GRU & 87.00 & 90.15 & 83.59 & 78.69 & 84.51 & 71.87 & 82.69 & 83.37 \\
      MDETR~\cite{kamath2021mdetr} & ENB3 & RoBERTa-base & 87.51 & 90.40 & 82.67 & 81.13 & 85.52 & 72.96 & 83.35 & 83.31\\
      OFA-B~\cite{wang2022ofa} & RN101 & 
      Embedding layer &  88.48 & 90.67 & 83.30 & 81.39 & 87.15 & 74.29 & 82.29 & 82.31 \\
    UniTAB~\cite{yang2022unitab} & RN101 & RoBERT-base & 88.59 & 91.06 & 83.75 & 80.97 & 85.36 & 71.55 & 84.58 & 84.70 \\
      % OFA-L~\cite{wang2022ofa} & RN152 & Embedding layer & 90.05 & \textbf{92.93} & 85.26 & \textbf{85.80} & \textbf{89.87} & \textbf{79.22} & 85.89 & \textbf{86.55} \\
      PolyFormer-L & Swin-L & BERT-base & 90.38 & 92.89 & 87.16 & 84.98 & 89.77 & 77.97 & 85.83 & 85.91 \\
      \hline

      \rowcolor{lightgray!28}\modelname-R50 & RN50 & RoBERTa-base & 87.37 & 90.33 & 84.04 & 77.36 & 83.08 & 69.50 & 81.25 & 82.47 \\
      \rowcolor{lightgray!28}\textbf{\modelname-L} & Swin-L & RoBERTa-base & \textbf{90.95} & 92.66 & \textbf{87.52} & 82.07 & 87.51 & 75.62 & \textbf{86.40} & 86.23 \\

      \bottomrule[1pt]
\end{tabular}
